Learning Hybrid Control Barrier Functions from Data

Motivated by the lack of systematic tools to obtain safe control laws for hybrid systems, we propose an optimization-based framework for learning certifiably safe control laws from data. In particular, we assume a setting in which the system dynamics are known and in which data exhibiting safe system behavior is available. We propose hybrid control barrier functions for hybrid systems as a means to synthesize safe control inputs. Based on this notion, we present an optimization-based framework to learn such hybrid control barrier functions from data. Importantly, we identify sufficient conditions on the data such that feasibility of the optimization problem ensures correctness of the learned hybrid control barrier functions, and hence the safety of the system. We illustrate our findings in two simulations studies, including a compass gait walker.

==> chapter/background.tex <==
\section{Preliminaries and Problem Formulation}
\label{sec:backgound}

%Let $\mathbb{R}$, $\mathbb{R}_{\ge 0}$, and $\mathbb{N}$ be the set of real, non-negative real, and natural numbers, while $\mathbb{R}^n$ is the $n$-dimensional real-valued vector space. 

\emph{Notation: }Let $\text{dom}(z):=\{(t,j)\in \mathbb{R}_{\ge 0}\times\mathbb{N}| \exists \zeta\in\mathbb{R}^{n_z} \text{ s.t. } z(t,j)=\zeta\}$ be the domain of a function $z:\mathbb{R}_{\ge 0}\times\mathbb{N}\to  \mathbb{R}^{n_z}$. A function $\alpha:\mathbb{R}\to\mathbb{R}$ is an extended class $\mathcal{K}$ function if $\alpha$ is strictly increasing and $\alpha(0)=0$. For $\epsilon>0$ and $p\ge 1$, let $\mathcal{B}_{\epsilon,p}(x_i):=\{x\in\mathbb{R}^n\, \big{|}\, \|x-x_i\|_p\le \epsilon\}$ be the closed $p$-norm ball around $x_i\in\mathbb{R}^n$. Let bd$(\mathcal{C})$ and int$(\mathcal{C})$ be the boundary and interior of a set $\mathcal{C}$. 

\subsection{Control Barrier Functions}
\label{sec:cbf}
At time $t\in\mathbb{R}_{\ge 0}$, let $x(t)\in\mathbb{R}^n$ and $u(t)\in\mathbb{R}^m$ be the state and input, respectively, of the dynamical control system  described by the initial value problem
\begin{align}\label{eq:system}
\dot{x}(t)=f(x(t))+g(x(t))u(t), \; x(0)\in\mathbb{R}^n
\end{align}
where $f:\mathbb{R}^n\to\mathbb{R}^n$ and $g:\mathbb{R}^n\to\mathbb{R}^{n\times m}$ are continuous functions. Let the solutions to \eqref{eq:system} under a continuous control law $u:\mathbb{R}^n\to\mathbb{R}^m$ be $x:\mathcal{I}\to \mathbb{R}^n$ where $\mathcal{I}\subseteq\mathbb{R}_{\ge 0}$ is the maximum definition interval of $x$. We do not assume forward completeness of \eqref{eq:system} under $u$ here, i.e., $\mathcal{I}$ may be bounded.

Consider next a continuously differentiable function $h:\mathbb{R}^n\to\mathbb{R}$ and define the set 
\begin{align*}
\mathcal{C}:=\{x\in\mathbb{R}^n \, \big{|} \, h(x)\ge 0\},
\end{align*}
which defines a set that we wish to certify as safe, i.e., that it satisfies prescribed safety specifications and can be made forward invariant through an appropriate choice of control action. Note that $\mathcal{C}$ is closed and further assume that $\mathcal{C}$ is not the empty set. Now, let $\mathcal{D}$ be an open set that is such that $\mathcal{D}\supseteq \mathcal{C}$. The function $h(x)$ is said to be a \emph{valid control barrier function} on $\mathcal{D}$ if there exists a locally Lipschitz continuous extended class $\mathcal{K}$ function $\alpha:\mathbb{R}\to\mathbb{R}$ such that 
\begin{align}\label{eq:cbf_const}
\sup_{u\in \mathcal{U}} %\frac{\partial \cbf(\xx)}{\partial \xx}
\langle \nabla h(x), f(x)+g(x)u\rangle \ge -\alpha(h(x))
\end{align} 
holds for all $x\in\mathcal{D}$, where $\mathcal{U}\in\mathbb{R}^n$ defines constraints on the control input $u$. Consequently, we define the set of \emph{CBF consistent inputs} induced by a valid CBF $h(x)$ to be 
\[
K_{\text{CBF}}(x):=\{u\in\mathbb{R}^m \, \big{|} \, %\frac{\partial \cbf(\xx)}{\partial \xx}
\langle \nabla h(x), f(x)+g(x)u\rangle \ge -\alpha(h(x))\}.\]

The next result follows mainly from \citet{ames2017control}. We provide a slightly modified version to account for  \citet[Remark 5]{ames2019control} and to not need to require that $\nabla h(x)\neq 0$ when $x\in \text{bd}(\mathcal{C})$. The proof uses the Comparison Lemma \citep[Lemma 3.4]{Kha96} and is given in the appendix.
\begin{lemma}\label{lem:1}
Assume that $h(x)$ is a valid control barrier function on $\mathcal{D}$ and that $u:\mathcal{D}\to \mathcal{U}$ is a continuous function with $u(x)\in K_{\text{CBF}}(x)$. Then $x(0)\in\mathcal{C}$ implies $x(t)\in\mathcal{C}$ for all $t\in \mathcal{I}$. If $\mathcal{C}$ is compact, it follows that $\mathcal{C}$ is forward invariant under $u(x)$, i.e., $\mathcal{I}=[0,\infty)$.
\end{lemma}

%Moreover, it holds that $\mathcal{C}$ is asymptotically stable under $u(x)$ when $\mathcal{C}$ is compact, which implies that $x(t)$ approaches $\mathcal{C}$ as $t\to\infty$ when $x(0)\in\mathcal{C}^c \cap \mathcal{D}$.
\subsection{Hybrid Systems }
\label{sec:RRSTL}

Hybrid systems are here modeled and analyzed in the framework of \citet{goebel2012hybrid,goebel2009hybrid}.

\begin{definition}\label{def:hybrid_system}
	A hybrid system \citep{goebel2012hybrid} is a tuple $\mathcal{H}:=(C,F,D,G)$ where $C\subseteq\mathbb{R}^{n_z}$, $D\subseteq\mathbb{R}^{n_z}$, $F:\mathbb{R}^{n_z}\to \mathbb{R}^{n_z}$, and $G:\mathbb{R}^{n_z}\to\mathbb{R}^{n_z}$ are the flow and jump sets and the continuous flow and jump maps, respectively. At the hybrid time $(t,j)\in \mathbb{R}_{\ge 0}\times\mathbb{N}$, let $z(t,j)\in \mathbb{R}^{n_z}$ be the hybrid state with initial condition $z(0,0)\in C\cup D$ and the hybrid system dynamics
	\begin{align}\label{eq:hybrid_systems}
	\begin{cases}
	\dot{z}(t,j)= F(z(t,j)) & \text{ }z(t,j) \in C  \\
	z(t,j+1)= G(z(t,j)) & \text{ }z(t,j) \in D. 
	\end{cases}
	\end{align}
\end{definition}

 Solutions to \eqref{eq:hybrid_systems} are parametrized by $(t,j)$, where $t$ indicates continuous \emph{flow} according to $F(z)$ and $j$ indicates \emph{jumps} according to $G(z)$. Let now $\mathcal{E} \subseteq \mathbb{R}_{\ge 0}\times \mathbb{N}$ be a \emph{hybrid time domain} \citep[Ch. 2.2]{goebel2012hybrid}, i.e., $\mathcal{E}$ is an infinite union of intervals of the form $[t_j,t_{j+1}]\times \{j\}$ or a finite union of intervals of the form $[t_j,t_{j+1}]\times \{j\}$ where the last interval, if existent, has the form $[t_j,t_{j+1}]\times \{j\}$, $[t_j,t_{j+1})\times \{j\}$, or $[t_j,\infty)\times \{j\}$. We now define a \emph{hybrid solution} $z:\mathcal{E}\to C\cup D$ to $\mathcal{H}$ formally as follows.

\begin{definition}\label{def:hybrid_solutions}
	A function $z:\mathcal{E}\to  C \cup D$ is a hybrid solution to $\mathcal{H}$ if $z(0,0)\in C \cup D$ and 
	\begin{itemize}
	    \item for each $j\in\mathbb{N}$ such that $I_j:= \{t\in\mathbb{R}_{\ge 0}|(t,j)\in \text{dom}(z) \}$ is not a singleton, $z(t,j)\in C$ and  $\dot{z}(t,j)=F(z(t,j))$ for all $t\in[\min I_j, \sup I_j)$
	    \item for each $(t,j)\in\text{dom}(z)$ s.t. $(t,j+1)\in\text{dom}(z)$, $z(t,j)\in D$ and $z(t,j+1)=G(z(t,j))$.
	\end{itemize}
\end{definition}



\begin{example}\label{ex:1}
Consider the bouncing ball example from \citet[Example 1.1]{goebel2012hybrid}. Let $x\in\mathbb{R}$ be the (vertical) position and $v\in\mathbb{R}$ be the (vertical) velocity of a point mass. Let $z:=\begin{bmatrix}x & v \end{bmatrix}^T$ and 
\begin{align*}
\begin{cases}
\dot{z}(t,j)= \begin{bmatrix} v(t,j) & - \gamma \end{bmatrix}^T & \text{ }z(t,j) \in C  \\
z(t,j+1)= \begin{bmatrix} x(t,j) & - \kappa v(t,j) \end{bmatrix}^T & \text{ }z(t,j) \in D
\end{cases}
\end{align*}
where $\gamma>0$ (gravity), $\kappa\in(0,1)$ (damping), $C:=\{z\in\mathbb{R}^2|x>0 \text{ or } x=0,v\ge 0\}$, and $D:=\{z\in\mathbb{R}^2|x=0,v<0\}$. For an initial condition $z(0,0):=\begin{bmatrix}x(0,0) & v(0,0) \end{bmatrix}^T$ with $x(0,0)> 0$, the hybrid time domain $\mathcal{E}$ is an infinite union of intervals of the form $[t_j,t_{j+1}]\times \{j\}$ where, as $j\to \infty$, $t_j$ converges to some constant value and where $\|z(t,j)\|$ converges to zero. 
\end{example}


	
\subsection{Problem Formulation}
The class of \emph{hybrid control systems} that we consider is
\begin{align}\label{eq:hybrid_control_systems}
\begin{cases}
\dot{z}(t,j)= f_c(z(t,j))+g_c(z(t,j))u_c(t,j) & \hspace{-0.3cm}z(t,j) \in C  \\
z(t,j+1)= f_d(z(t,j))+g_d(z(t,j))u_d(t,j) & \hspace{-0.3cm}z(t,j) \in D
\end{cases}
\end{align}
where $u_c(t,j)\in \mathbb{R}^{m_c}$ and $u_d(t,j)\in\mathbb{R}^{m_d}$ are the control inputs during flows and jumps, respectively. Let $f_c:\mathbb{R}^{n_z}\to\mathbb{R}^{n_z}$, $f_d:\mathbb{R}^{n_z}\to\mathbb{R}^{n_z}$, $g_c:\mathbb{R}^{n_z}\to\mathbb{R}^{n_z\times n_c}$, and $g_d:\mathbb{R}^{n_z}\to\mathbb{R}^{n_z\times m_d}$ be continuous functions and $u_c:\mathcal{D}_C\to \mathbb{R}^{m_c}$ and $u_d:\mathcal{D}_D\to \mathbb{R}^{m_d}$ be  continuous control laws defined on the sets $\mathcal{D}_C\subseteq C$ and $\mathcal{D}_D\subseteq D$. The sets $\mathcal{D}_C$ and $\mathcal{D}_D$ are the equivalent to the set $\mathcal{D}$ in Section \ref{sec:cbf}, but now considered separately for flows and jumps.  Let  hybrid solutions to the system \eqref{eq:hybrid_control_systems} under continuous control laws $u_c:\mathcal{D}_C\to \mathbb{R}^{m_c}$ and $u_d:\mathcal{D}_D\to \mathbb{R}^{m_d}$ hence be $z:\mathcal{E}\to \mathcal{D}_C\cup \mathcal{D}_D$.\footnote{We again do not assume completeness of the system \eqref{eq:hybrid_control_systems} under $u_c$ and $u_d$. Completeness here means that the hybrid time domain $\text{dom}(z)$ is unbounded (see \citet[Ch. 2.2]{goebel2012hybrid} for a formal definition).}


We are additionally given a set of \emph{expert trajectories} consisting of $N_c$ and $N_d$ discretely sampled data-points along flows and jumps as $Z_\text{dyn}^c:=\{(z^i,u^i_c)\}_{i=1}^{N_c}$ for $z^i\in C$ and $Z_\text{dyn}^d:=\{(z^i,u^i_d)\}_{i=1}^{N_d}$ for $z^i\in D$, as illustrated in Figure \ref{fig:1} (left).\footnote{We refer to the collection of data points $Z_\text{dyn}^c$ and $Z_\text{dyn}^d$ as expert trajectories  to emphasize that this is a natural way of collecting the $\{(z^i,u_c^i)\}$ and $\{(z^i,u_d^i)\}$ pairs from the system \eqref{eq:hybrid_control_systems}.  We note, however, that our method simply requires a collection of state-action pairs $\{(z^i,u_c^i)\}$ and $\{(z^i,u_d^i)\}$ demonstrating safe behavior.} It is assumed that each $z^i\in\text{int}(\mathcal{S})$ where $\mathcal{S}\subseteq \mathbb{R}^{n_z}$ is referred to as the \emph{geometric safe set}, i.e., the set of safe states. 

Our goal is now to learn, from $Z_\text{dyn}^c$ and $Z_\text{dyn}^d$,  a differentiable function $h:\mathbb{R}^{n_z}\to\mathbb{R}$ such that
\begin{align}\label{eq:set_C}
\mathcal{C}:=\{z\in\mathbb{R}^{n_z} \, \big{|} \, h(z)\ge 0\}
\end{align}
can be made forward invariant by appropriate control actions $u_c(z)$ and $u_d(z)$ and with $\mathcal{C}\subseteq \mathcal{S}$, i.e., the set $\mathcal{C}$ that is defined based on the learned HCBF under-approximates the geometric safe set $\mathcal{S}$. 

%which we again assume to have non-empty interior. 
%So far, only hybrid barrier functions for safety verification have been considered in the literature.  In this paper we: 1) propose hybrid control barrier functions, 2) present an optimization-based framework to learn such hybrid control barrier functions from expert trajectories, and 3) provide verifiable conditions under which the learned hybrid control barrier functions guarantees safe trajectories. 



==> chapter/control_strategy.tex <==
\section{Proposed Problem Solution}


\subsection{Hybrid Control Barrier Functions}
Let $h:\mathbb{R}^{n_z}\to\mathbb{R}$ be a continuously differentiable function for which the set $\mathcal{C}$ in \eqref{eq:set_C} is not empty. 

\begin{assumption}\label{ass:1}
The closed set $\mathcal{C}$ defined in \eqref{eq:set_C} is contained within the set $C\cup D$, i.e., $\mathcal{C}\subseteq C\cup D$. 
\end{assumption} 

Assumption \ref{ass:1} is not restrictive and natural since we are only interested in regions where the system \eqref{eq:hybrid_control_systems} is defined. Consider now the sets $\mathcal{D}_C\subseteq \mathbb{R}^{n_z}$ and $\mathcal{D}_D\subseteq \mathbb{R}^{n_z}$ that are such that $\mathcal{C}\cap C \subseteq \mathcal{D}_C$ and $\mathcal{C}\cap D \subseteq\mathcal{D}_D$ so that $\mathcal{C}\subseteq \mathcal{D}_C\cup \mathcal{D}_D$\footnote{This follows since $\mathcal{C}\subseteq C\cup D$ (Assumption \ref{ass:1}) results in $(\mathcal{C}\cap C)\cup(\mathcal{C}\cap D)=\mathcal{C} \cap (C\cup D)=\mathcal{C}$ and since $(\mathcal{C}\cap C)\cup(\mathcal{C}\cap D)\subseteq \mathcal{D}_C\cup \mathcal{D}_D$ by the choices of the sets $\mathcal{D}_C$ and $\mathcal{D}_D$. }, which ensures that the set $\mathcal{D}:=\mathcal{D}_C\cup\mathcal{D}_D$ fully covers $\mathcal{C}$. 



\begin{definition}
The function $h(z)$ is said to be a \emph{valid hybrid control barrier function}  on $\mathcal{D}$ if 
\begin{itemize}
    \item there exists a locally Lipschitz continuous extended class $\mathcal{K}$ function $\alpha:\mathbb{R}\to \mathbb{R}$ such that 
    \begin{align}\label{eq:cbf_const_hybrid}
        \sup_{u_c\in \mathcal{U}_c} %\frac{\partial \cbf(\xx)}{\partial \xx}
        \langle \nabla h(z), f_c(z)+g_c(z)u_c\rangle \ge -\alpha(h(z))
    \end{align} 
    holds for all $z\in \mathcal{D}_C$, where $\mathcal{U}_c\in\mathbb{R}^{m_c}$ defines constraints on the  control input $u_c$.
    \item it holds that 
    \begin{align}\label{eq:cbf_disc_hybrid}
        \sup_{u_d\in \mathcal{U}_d} h(f_d(z)+g_d(z)u_d) \ge 0 
    \end{align}
    for all $z\in \mathcal{D}_D$, where $\mathcal{U}_d\in\mathbb{R}^{m_d}$ defines constraints on the  control input $u_d$.
\end{itemize}
\end{definition}

Based on the above definition, let us next define the sets of HCBF consistent inputs to be
\[
K_{\text{HCBF},c}(z):=\{u_c\in\mathcal{U}_c\, \big{|} \, %\frac{\partial \cbf(\xx)}{\partial \xx}
\langle \nabla h(z), f_c(z)+g_c(z)u_c\rangle \ge -\alpha(h(z))\}\]
\[
K_{\text{HCBF},d}(z):=\{u_d\in\mathcal{U}_d\, \big{|} \, %\frac{\partial \cbf(\xx)}{\partial \xx}
 h(f_d(z)+g_d(z)u_d) \ge 0\}.\]
 
 Assume for the remainder that the set $\mathcal{D}_C$ is open.\footnote{If $\mathcal{D}_C$ is not open, one can instead assume that $\mathcal{C}\setminus \mathcal{D}_D$ is strictly contained within $\mathcal{D}_C\cup \mathcal{D}_D$.} This will allow us, in the next result, to establish forward invariance of the set $\mathcal{C}$ under control laws $u_c(z)$ and $u_d(z)$  when the set $\mathcal{C}$ is compact. 
\begin{theorem}\label{thm:1}
Assume that $h(z)$ is a valid hybrid control barrier function on $\mathcal{D}$ and that $u_c:\mathcal{D}_C\to \mathcal{U}_c$ and $u_d:\mathcal{D}_D\to \mathcal{U}_d$ are continuous functions with $u_c(z)\in K_{\text{HCBF},c}(z)$ and $u_d(z)\in K_{\text{HCBF},d}(z)$. Then $z(0,0)\in\mathcal{C}$ implies $z(t,j)\in\mathcal{C}$ for all $(t,j)\in \text{dom}(z)$. If $\mathcal{C}$ is compact and Assumption \ref{ass:1} holds, it follows that $\mathcal{C}$ is forward invariant under $u_c(z)$ and $u_d(z)$, i.e., $\text{dom}(z)$ is unbounded.

\begin{proof}
The proof is based on showing that both during flows and jumps $h(t,j)\ge 0$ due to the constraints \eqref{eq:cbf_const_hybrid} and \eqref{eq:cbf_disc_hybrid}. Showing that the hybrid time domain $\text{dom}(z)$ is unbounded relies on showing that $z(t,j)$ can not leave $\mathcal{D}_C\cup\mathcal{D}_D$. The complete proof is given in the appendix.
 %$z(t,j)$ can be extended by flowing, either by flowing into $\mathcal{D}_D\cap \mathcal{C}$ or by flowing within $\mathcal{C}\setminus \mathcal{D}_D\cap \mathcal{C}$. . Hence, by contradiction, it holds that $\mathcal{E}$ is unbounded. 
 %Since the set $\mathcal{D}_C$ is open, we can now always extend a solution within $\mathcal{C}$, for $z\in \mathcal{C}\setminus \mathcal{D}_D$ by flowing and for $z\in \mathcal{D}_D \cap \mathcal{C}$ in particular by jumping (even though flowing may also be possible). During flows and similar to the proof of Lemma \ref{lem:1}, it holds that solutions exist until (if at all) a jump occurs since $\mathcal{C}$ is compact and due to Assumption \ref{ass:2}. After jumps, $z(t_{j+1},j+1)\in \mathcal{C}\subseteq \mathcal{D}_C\cup \mathcal{D}_D$, which ensures that a continuation of the solution always exists and the domain $\mathcal{E}$ is unbounded by \citet[Proposition 2.10]{goebel2012hybrid}.
 \end{proof}
\end{theorem}

\begin{example}\label{ex:2}
Consider again the bouncing ball example from Example \ref{ex:1}, here equipped with continuous and discrete control inputs as an academic and easy to follow example. The dynamics are
\begin{align*}
\begin{cases}
\dot{z}(t,j)= \begin{bmatrix} v(t,j) & u_c- \gamma \end{bmatrix}^T & \text{ }z(t,j) \in C  \\
z(t,j+1)= \begin{bmatrix} x(t,j) & - u_dv(t,j) \end{bmatrix}^T & \text{ }z(t,j) \in D
\end{cases}
\end{align*}
and the geometric safe set is $\mathcal{S}:=\{z\in\mathbb{R}^2| v^2\le \zeta\}$. Even though the control inputs $u_c$ and $u_d$ are artificially added, they can be thought of as controllable wind resistance and floor damping. Let us define the function $h(z):=\zeta-v^2$ so that $\mathcal{C}=\mathcal{S}$. With respect to \eqref{eq:cbf_const_hybrid} and for $\alpha(r):=r$, we get $\langle \nabla h(z), f_c(z)+g_c(z)u_c\rangle \ge -\alpha(h(z))$ which is equivalent to $ -2 v u_c+2v\gamma \ge  -\zeta+v^2$ and for which we can always find a suitable $u_c\in\mathbb{R}$. With respect to \eqref{eq:cbf_disc_hybrid}, we get $h(f_d(z)+g_d(z)u_d) \ge 0$ which is equivalent to $\zeta-(u_dv)^2 \ge 0$ and for which we can, again, always find a suitable $u_d\in\mathbb{R}$.
\end{example}

%\begin{example}
%Consider again the bouncing ball example from \citet[Example 1.1]{goebel2012hybrid}, here equipped with continuous and discrete inputs as an academic and easy to follow example. Let $x\in\mathbb{R}$ be the (vertical) position and $v\in\mathbb{R}$ be the (vertical) velocity of a point mass. Let $z:=\begin{bmatrix}x & v \end{bmatrix}^T$ and 
%\begin{align*}
%\begin{cases}
%\dot{z}(t,j)= \begin{bmatrix} v(t,j) & u_c- \gamma \end{bmatrix}^T & \text{ }z(t,j) \in C  \\
%z(t,j+1)= \begin{bmatrix} x(t,j) & - u_dv(t,j) \end{bmatrix}^T & \text{ }z(t,j) \in D
%\end{cases}
%\end{align*}
%where $\gamma>0$ (gravity), $C:=\{z\in\mathbb{R}^2|x>0 \text{ or } x=0,v\ge 0\}$, and $D:=\{z\in\mathbb{R}^2|x=0,v<0\}$. Let our geometric safe set be $\mathcal{S}:=\{z\in\mathbb{R}^2| \|v\|^2\le \zeta\}$ and let us define the function $h(z):=\zeta-\|v\|^2$ so that $\mathcal{C}=\mathcal{S}$. With respect to \eqref{eq:cbf_const_hybrid} and for $\alpha(r):=r$, we get $\langle \nabla h(z), f_c(z)+g_c(z)u_c\rangle \ge -\alpha(h(z))$ which is equivalent to $ -2 v u_c+2v\gamma \ge  -\zeta+\|v\|^2$ and for which we can always find a suitable $u_c\in\mathbb{R}$. With respect to \eqref{eq:cbf_disc_hybrid}, we get $h(f_d(z)+g_d(z)u_d) \ge 0$ which is equivalent to $\zeta-\|u_dv\|^2 \ge 0$ and for which we can, again, always find $u_d\in\mathbb{R}$ satisfying this inequality.
%\end{example}


\subsection{Learning Valid Hybrid Control Barrier Functions from Data}
\label{sec:compute}

\begin{figure*}
\centering
\includegraphics[scale=0.25]{1.eps}
\hspace{0.5cm}\includegraphics[scale=0.25]{2.eps}\hspace{0.5cm}\includegraphics[scale=0.25]{3.eps}
\caption{Problem setup (left): The flow and jump sets (blue and purple boxes) and the set of safe expert trajectories during flows and jumps (black lines and dots). Set definitions (middle): The sets $\mathcal{D}_C$ and $\mathcal{D}_D$ (black and light red balls) are the union of $\epsilon$ balls around the expert trajectories during flows and jumps. The set $\mathcal{N}$ (golden rings), defined around $\mathcal{D}_C$ and $\mathcal{D}_D$, ensures that the learned safe set $\mathcal{C}$ is such that $\mathcal{C}\subset\mathcal{D}\subseteq\mathcal{S}$. Note that the geometrical safe set $\mathcal{S}$ is not depicted here. Desired result (right): The learned safe set $\mathcal{C}$ (red region) is defined via the learned valid HCBF $h(z)$.}
\label{fig:1}
\end{figure*}
First, define the sets $Z_\text{safe}^c := \{ z^i : (z^i, u^i_c) \in Z_\text{dyn}^c \}$ and $Z_\text{safe}^d := \{ z^i : (z^i, u^i_d) \in Z_\text{dyn}^d \}$. Towards the goal of learning a valid HCBF, we now define, for $\epsilon_c,\epsilon_d>0$ and $p\ge 1$, the data sets
\begin{align}\label{eq:set_D}
    \mathcal{D}_D:=D\cap\bigcup_{z^i\in Z_\text{safe}^d}\mathcal{B}_{\epsilon_d,p}(z^i) \,\text{ and }\, \mathcal{D}_C := \mathcal{D}_C' \backslash \mathrm{bd}(\mathcal{D}_C') \,\text{ where }\, \mathcal{D}_C'&:=C\cap \bigcup_{z^i\in Z_\text{safe}^c}\mathcal{B}_{\epsilon_c,p}(z^i).
\end{align} 
Note that the set $\mathcal{D}_C $ is open by definition. For $\sigma>0$, define
\begin{align*}
    \mathcal{N}&:= \{\text{bd}(\mathcal{D})\oplus\mathcal{B}_{\sigma,p}(0)\} \setminus \mathcal{D},
\end{align*} 
where $\mathcal{N}$ is a ring of diameter $\sigma$ that surrounds the set $\mathcal{D}$ (see the golden ring in Figure \ref{fig:1}). We will use the set $\mathcal{N}$ to enforce that the value of the learned HCBF $h(z)$ is negative on $\mathcal{N}$ to ensure that the set $\mathcal{C}$ is contained within the set $\mathcal{D}$, which is a necessary condition for $h(z)$ to be valid. Hence, also assume that points $Z_N = \{z^i\}_{i=1}^{\bar{N}}$ are sampled from $\mathcal{N}$, i.e., $z^i\in \mathcal{N}$.  Note that only state space data points $z^i\in Z_N$ are sampled from $\mathcal{N}$, while no input samples $u_c^i$ or $u_d^i$ need to be obtained. While the set $\mathcal{C}$ defined in \eqref{eq:set_C} considers all $z\in \mathbb{R}^{n_z}$ such that $h(z) \geq 0$, we modify this definition slightly by restricting the domain to set $\mathcal{N} \cup \mathcal{D}$. This restriction is natural since we are learning a HCBF $h(z)$ from data sampled only over the domain $\mathcal{N} \cup \mathcal{D}$. Let us hence define the set
\begin{align} \label{eq:local_C}
\mathcal{C}:=\{z\in\mathcal{N} \cup \mathcal{D}\, \big{|} \, h(z)\ge 0\}
\end{align}
and consider to learn a valid \emph{local} HCBF $h(z)$  on $\mathcal{D}$ with respect the set $\mathcal{C}$ defined in \eqref{eq:local_C}.


\textbf{The optimization problem: }We now propose the optimization problem that allows to learn a valid local HCBF and prove its correctness afterwards. We solve
\begin{subequations}\label{eq:opt}
\begin{align}
    &\min_{h \in \mathcal{H}} \:\: \|h\|   \: \nonumber \\
    &\mathrm{s.t.}~~ h(z^i) \geq \gamma_\text{safe}, \: \forall z^i \in Z_\text{safe}^c\cup Z_\text{safe}^d \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{: safe set with margin $\gamma_\text{safe}>0$}\label{eq:cons_1}\\
    &~~~~~~ h(z^i) \leq -\gamma_\text{unsafe}, \: \forall z^i \in Z_N \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;  \text{: unsafe set with margin $\gamma_\text{unsafe}>0$}  \label{eq:cons_2}\\
    &~~~~~~ \text{Lip}(h(z^i),\bar{\epsilon}) \leq L_h, \: \forall z^i \in Z_N \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;  \text{: Lipschitz constraint on $h(z)$}  \label{eq:lip1}\\
    &~~~~~~  q_c(z^i,u^i_c):=\langle\nabla h(z^i), f_c(z^i)+g_c(z^i) u^i_c) \rangle + \alpha(h(z^i)) \geq \gamma_\text{dyn}^c \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{: derivative}  \label{eq:cons_3}\\
    &\hspace{7cm}\;\;\;\;\;\;\;\;\; \text{constraint \eqref{eq:cbf_const_hybrid} with margin $\gamma_\text{dyn}^c>0$}\nonumber\\
    &~~~~~~ \text{Lip}(q_c(z^i,u^i_c),\epsilon_c) \leq L_q^c, \: \forall (z^i, u^i_c) \in Z_\text{dyn}^c \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{: Lipschitz constraint on $q_c(z,u^i_c)$} \label{eq:lip2_c}\\
     &~~~~~~  q_d(z^i,u^i_d):= h( f_d(z^i)+g_d(z^i) u^i_d) \geq \gamma_\text{dyn}^d \;\;\; \text{: jump constraint \eqref{eq:cbf_disc_hybrid} with margin $\gamma_\text{dyn}^d>0$} \label{eq:cons_4}\\
    &~~~~~~ \text{Lip}(q_d(z^i,u^i_d),\epsilon_d) \leq L_q^d, \: \forall (z^i, u^i_d) \in Z_\text{dyn}^d  \;\;\;\;\;\;\;\;\;\;\;\;\;\;\, \text{: Lipschitz constraint on $q_d(z,u^i_d)$}\label{eq:lip2_d}
\end{align}
\end{subequations}
%Here $\lambda>0$ is a regularization weight, and we slightly abuse notation and let $f(x, u) = f(x) + g(x) u$.

where $\mathcal{H}$ is a symmetric normed function space and where the positive constants $\gamma_\text{safe}$, $\gamma_\text{unsafe}$, $\gamma_\text{dyn}^c$,$\gamma_\text{dyn}^d$, $L_h$, $L_q^c$, and $L_q^d$  are
\emph{hyperparameters} that are set according to the data-sets $Z_\text{safe}^c$, $Z_\text{safe}^d$, and $Z_N$ that have to be sampled ``dense'' enough, as quantified by $\bar{\epsilon}$, $\epsilon_c$, and $\epsilon_d$ (conditions given below). The constraints in \eqref{eq:lip1}, \eqref{eq:lip2_c}, and \eqref{eq:lip2_d} assume that there exists a function $\text{Lip}(\cdot,\epsilon)$ that returns an upper bound on the Lipschitz constant of its argument with respect to the state $z$ in an $\epsilon$ neighborhood of $z^i$ using the $p$-norm (more details below). It may be difficult to enforce the constraints \eqref{eq:lip1}, \eqref{eq:lip2_c}, and \eqref{eq:lip2_d} in the optimization problem \eqref{eq:opt}. One can resort to bootstrapping the values of $L_h$, $L_q^c$, and $L_q^d$ by iteratively solving the optimization problem \eqref{eq:opt} and calculating the values of $L_h$, $L_q^c$, and $L_q^d$ in order to verify if the constraints \eqref{eq:lip1}, \eqref{eq:lip2_c}, and \eqref{eq:lip2_d} hold. If not, the hyperparameters can be adjusted accordingly. If we hence solve the optimization problem \eqref{eq:opt} without the constraints \eqref{eq:lip1}, \eqref{eq:lip2_c}, and \eqref{eq:lip2_d}, we can observe that \eqref{eq:opt} is convex in $h$ if $\alpha(\cdot)$ is a linear function. If $\mathcal{H} := \{ h_\theta(z) = \langle \phi(z), \theta \rangle | \theta \in \Theta \}$
where $\Theta$ is a convex set and where $\phi:\mathbb{R}^{n_z}\to\mathbb{R}$ is a known function, then the optimization problem~\eqref{eq:opt} is convex in $\theta$. In the more general case, i.e., $\mathcal{H} := \{ h(z; \theta) | \theta \in \Theta \}$, as for instance when $h(z)$ is a deep neural net, \eqref{eq:opt} becomes a nonconvex optimization problem for which we propose, similarly to \citet{robey2020learning}, an unconstrained
relaxation that can be solved efficiently. Let $[r]_+ := \max \{r, 0\}$ for $r\in\mathbb{R}$ and solve instead of the constrained optimization problem \eqref{eq:opt} the unconstrained optimization problem
\begin{align*}
    &\min_{\theta \in \Theta} ~~ \|\theta\|^2 + \lambda_{\mathrm{s}} \sum_{z^i \in Z_\text{safe}^c\cup Z_\text{safe}^d} [\gamma_\text{safe} - h_\theta(z^i)]_+ 
    + \lambda_{\mathrm{u}} \sum_{z^i \in Z_N} [h_\theta(z^i) + \gamma_\text{unsafe}]_+ +\lambda_{\mathrm{d}} \sum_{(z^i, u^i_c) \in Z_\text{dyn}^c} [\gamma_\text{dyn}^c  \\
    & -  \langle \nabla h_\theta(z^i), f_c(z^i)+g_c(z^i)u_c^i \rangle - \alpha(h_\theta(z^i)) ]_+ + \lambda_{\mathrm{c}} \sum_{(z^i, u^i_d) \in Z_\text{dyn}^d} [\gamma_\text{dyn}^d -  h_\theta(f_d(z^i)+g_d(z^i)u_d^i) ]_+  \:.
\end{align*}
where $\lambda_{\mathrm{s}}, \lambda_{\mathrm{u}},\lambda_{\mathrm{d}},\lambda_{\mathrm{c}}>0$ allow to trade off the constraints \eqref{eq:cons_1}, \eqref{eq:cons_2}, \eqref{eq:cons_3}, and \eqref{eq:cons_4}. While the proposed unconstrained optimization problem is still non-convex, we can solve it efficiently with stochastic first-order gradient methods
such as Adam or stochastic gradient descent. 

At this point, some remarks are in place. The set $Z_N$ can simply be obtained by gridding or uniform sampling of the set $\mathcal{D}$ (see \citet[Section 3.5]{robey2020learning} for a discussion). The sets $Z_\text{dyn}^c$ and $Z_\text{dyn}^d$ should contain state input pairs $(z^i,u_c^i)$ and $(z^i,u_d^i)$ that illustrate safe system behavior by illustrating how to move from the boundary of $\mathcal{S}$ inside of $\mathcal{S}$. For the derivative constraint in \eqref{eq:cons_3} this means to show behavior where the gradient $\nabla h(z^i)$ is not perpendicular to the control direction $g_c(z^i)u_c^i$, while for the jump constraint in \eqref{eq:cons_3} this means that the control term $g_d(z^i)u_d^i$ should not be zero. To verify \eqref{eq:lip1}, \eqref{eq:lip2_c}, and \eqref{eq:lip2_d}, Lipschitz constants of $h(z)$ as well as of $\nabla h(z)$ need to be obtained on which a discussion can be found in \citet[Section 3.4.2]{robey2020learning}. Using these Lipschitz constants, it can be seen that the functions $q_c(z^i,u_c^i)$ and $q_d(z^i,u_d^i)$ in \eqref{eq:cons_3} and \eqref{eq:cons_4} are Lipschitz continuous in $z$ since $\nabla h(z)$, $f_c(z)$, $f_d(z)$, $g_c(z)$, $g_d(z)$, and $\alpha(h(z))$ are Lipschitz continuous and since function composition preserves Lipschitz continuity \citep[Ch. 12]{eriksson2013applied}. 



In the remainder, we show correctness of the learned HCBF $h(z)$  obtained from \eqref{eq:opt} in two steps by: 1) showing that $\mathcal{C}\subset \mathcal{D}\subseteq \mathcal{S}$, and 2) proving that $h(z)$ is a valid local HCBF, ensuring that the set $\mathcal{C}$ can be made forward invariant by appropriate control laws $u_c(z)$ and $u_d(z)$.



\textbf{1) Guaranteeing $\mathcal{C}\subset \mathcal{D}\subseteq \mathcal{S}$: } We assume now that the unsafe samples $Z_N$ form an $\bar{\epsilon}$-net of $\mathcal{N}$, i.e., for all $z \in \mathcal{N}$,  there exists $z^i\in Z_N$ such that $\|z^i-z\|_p\leq \bar{\epsilon}$. Consider now the constraint \eqref{eq:cons_2} for which we derive conditions so that the learned HCBF satisfies $h(z) < 0$ for all $z \in \mathcal{N}$.

\begin{proposition}\label{prop:1}
Let $h(z)$ be Lipschitz continuous with local constant $L_h(z)$\footnote{By local constant, we here mean a Lipschitz constant in an $\bar{\epsilon}$ neighborhood of $z$.}, $\gamma_\text{unsafe}>0$ and $Z_N $ be an $\bar{\epsilon}$-net of $\mathcal{N}$ with $\bar{\epsilon}<\gamma_\text{unsafe}/L_h(z^i)$ for all $z^i \in Z_N$. Then, \eqref{eq:cons_2} ensures $h(z)<0$ for all $z\in\mathcal{N}$.
%, and consequently, $\C\subseteq\D\subseteq \Ss$.

\begin{proof}
This proof follows from an $\bar{\epsilon}$-net covering and Lipschitz continuity argument, similarly to \citet[Proposition 3.1]{robey2020learning}. The complete proof is given in the appendix.
\end{proof}
\end{proposition}

Consider next the constraint \eqref{eq:cons_1} which ensures that the set $\mathcal{C}$ over which $h(z)\geq 0$, as defined in equation \eqref{eq:local_C}, has non-empty interior. The next result follows in the same way as Proposition \ref{prop:1} and guarantees, together with Proposition \ref{prop:1}, that $\mathcal{C}\subset\mathcal{D}\subseteq\mathcal{S}$.
\begin{corollary}\label{cor:1}
Let $h(z)$ be Lipschitz continuous with local constant $L_h(z)$, $\gamma_\text{safe}>0$, and $Z_\text{safe}^c$ and $Z_\text{safe}^d$ be an ${\epsilon}_c$-net and an ${\epsilon}_d$-net of $\mathcal{D}_C$ and $\mathcal{D}_D$, respectively, with $\max({\epsilon}_c,{\epsilon}_d)\leq\gamma_\text{safe}/L_h(z^i)$ for all $z^i \in Z_\text{safe}^c\cup Z_\text{safe}^d$. Then, \eqref{eq:cons_1} ensures $h(z)\geq 0$ for all $z\in\mathcal{D}$.

\begin{proof}
The proof is similar to Proposition \ref{prop:1} and given in the appendix.
\end{proof}
\end{corollary}

Note that the constraints \eqref{eq:cons_1} and \eqref{eq:cons_2} may, in practice, lead to infeasibility of \eqref{eq:opt}. We resort to the same remedy as proposed in \citet[equation (3.4)]{robey2020learning}, i.e., enforcing \eqref{eq:cons_1} on smaller sets $\bar{Z}_\text{safe}^c$ and $\bar{Z}_\text{safe}^d$ with $\bar{Z}_\text{safe}^c\subset Z_\text{safe}^c$ and $\bar{Z}_\text{safe}^d\subset Z_\text{safe}^d$, respectively, to allow for smoother HCBFs to be learned at the expense of a smaller set $\mathcal{C}$.



\textbf{2) Guaranteeing valid local HCBF: } For $z\in \mathcal{D}_C$, define the function $q_c(z,u_c^i):= \langle \nabla h(z),f_c(z)+g_c(z)u^i_c\rangle+\alpha(h(z))$ where the control sample $u_c^i$ is associated with the sample $z^i$ that is such that $\|z^i-z\|_p\le \epsilon_c$. Note that such a pair $(z^i,u_c^i)\in Z_\text{dyn}^c$ is guaranteed to exist when the set $Z_\text{safe}^c$ is an $\epsilon_c$-net of $\mathcal{D}_D$. The function $q_c(z,u_c^i)$ is Lipschitz continuous in $z$ with local constant denoted by $L_q^c(z,u_c^i)$. Similarly, define $q_d(z,u_d^i):= h(f_d(z)+g_d(z)u^i_d)$ and note that $q_d(z,u_d^i)$ is Lipschitz continuous with local constant denoted by $L_q^d(z,u_d^i)$. We next provide conditions guaranteeing that the learned HCBF satisfies the constraint \eqref{eq:cbf_const_hybrid} for all $z \in \mathcal{D}_C$ and the constraint \eqref{eq:cbf_disc_hybrid} for all $z \in \mathcal{D}_D$.


\begin{proposition}\label{prop:2}
Suppose $q_c(z,u_c^i)$ and $q_d(z,u_d^i)$ are Lipschitz continuous with local constants $L_q^c(z,u_c^i)$ and $L_q^d(z,u_d^i)$, respectively.  Let $\gamma_\text{dyn}^c,\gamma_\text{dyn}^d>0$, and
\begin{enumerate}
    \item $Z_\text{safe}^c$ be an $\epsilon_c$-net of $\mathcal{D}_C$ with $\epsilon_c\leq \gamma_\text{dyn}^c/L_q^c(z^i,u_c^i)$ for all $(z^i,u_c^i)\in Z_\text{dyn}^c$
    \item $Z_\text{safe}^d$ be an $\epsilon_d$-net of $\mathcal{D}_D$ with $\epsilon_d\leq \gamma_\text{dyn}^d/L_q^d(z^i,u_d^i)$ for all $(z^i,u_d^i)\in Z_\text{dyn}^d$.
\end{enumerate} 

Then, \eqref{eq:cons_3} and \eqref{eq:cons_4} ensure that $q_c(z)\geq 0$ for all $z \in \mathcal{D}_C$ and $q_d(z)\geq 0$ for all $z \in \mathcal{D}_D$.
\begin{proof}
This proof follows from an $\epsilon_c$-net and an $\epsilon_d$ covering and Lipschitz continuity argument, similarly to \citet[Proposition 3.1]{robey2020learning}. The proof is given in the appendix.
\end{proof}
\end{proposition}

The next theorem summarizes the  results and guarantees that $h(z)$ from \eqref{eq:opt} is a valid HCBF.

\begin{theorem}\label{thm:2}
Let $h(z)$ be a continuously differentiable function and let the sets $\mathcal{S}$, $\mathcal{N}$, $\mathcal{D}_C$, $\mathcal{D}_D$, $\mathcal{D}$, $\mathcal{C}$, and the data-sets $Z_\text{dyn}^c$, $Z_\text{dyn}^d$, $Z_\text{safe}^c$, $Z_\text{safe}^d$, and $Z_N$ be defined as above. Suppose that $Z_N$ forms an $\bar{\epsilon}$-net of $\mathcal{N}$ satisfying the conditions of Proposition \ref{prop:1}, and that $Z_\text{safe}^c$ and $Z_\text{safe}^d$ are an ${\epsilon}_c$-net and an ${\epsilon}_d$-net of $\mathcal{D}_C$ and $\mathcal{D}_D$, respectively, satisfying the conditions of Corollary \ref{cor:1} \& Proposition \ref{prop:2}. Let $h(z)$, $q_c(z,u_c^i)$, and $q_d(z,u_c^i)$ be Lipschitz continuous with local constants $L_h(z)$, $L_q^c(z,u_c^i)$, and $L_q^d(z,u_d^i)$, respectively. Then if $h(z)$ satisfies constraints \eqref{eq:cons_1}, \eqref{eq:cons_2},\eqref{eq:cons_3}, and \eqref{eq:cons_4}, it holds that the set $\mathcal{C}$ is non-empty, $\mathcal{C}\subset\mathcal{D}\subseteq\mathcal{S}$, and the function $h(z)$ is a valid local hybrid control barrier function on $\mathcal{D}$ with domain $\mathcal{N} \cup \mathcal{D}$.
\end{theorem}





==> chapter/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Consider the following \emph{safety-critical} scenarios: autonomous vehicles in urban areas \citep{schwarting2018planning}, lower-body exoskeletons enabling disabled people to walk \citep{tucker2019preference}, and robots navigating through a warehouse according to higher-level logic \citep{kress2009temporal}. Despite being different in nature, these systems are inherently described by both continuous and discrete dynamics and states, i.e., \emph{hybrid}, either due to higher-level (logical) decision making or directly due to their physics. Importantly, these scenarios share the similarities that: 1) \emph{data} exhibiting safe behavior is readily available or can be collected, and 2) in most cases, their hybrid system dynamics are well understood and can be modeled/identified. Based on these observations, we propose an optimization-based framework to learn \emph{provably safe controllers} for hybrid systems based on a notion of \emph{hybrid control barrier functions} (HCBF). 



\textbf{Related work:} \emph{Barrier functions} have appeared in \citet{prajna2007framework} for certifying the safety of continuous-time systems. Nonsmooth and hybrid barrier functions were proposed in \citet{glotfelter2017nonsmooth,glotfelter2019hybrid}, respectively. Different to our work, the focus in the latter is on time-varying barrier functions with jumps for discontinuous systems.  \emph{Control barrier functions} (CBF) for continuous-time control systems have first appeared in \citet{wieland2007constructive} for synthesizing feedback control laws that ensure the safety of the system by ensuring forward invariance of a desired safe set.  Reciprocal and zeroing CBFs have been proposed in \citet{ames2014control,ames2017control}, respectively, and are less restrictive since no forward invariance of subsets of the safe set needs to be ensured. CBFs can then be used as a safety guard using convex quadratic programs \citep{ames2014control,ames2017control}, a feature that has been used for safe learning \citep{khojasteh2019probabilistic}. Robustness of CBF-based control laws has been analyzed in \citet{xu2015robustness}.   \emph{Discrete control barrier functions}, which are CBFs for discrete-time control systems, have appeared in \citet{agrawal2017discrete} and \citet{ohnishi2019barrier}. More related to this paper, \emph{hybrid barrier functions} were proposed in \citet{maghenem2019characterizations} and in \citet{bisoffi2018hybrid} in the hybrid systems framework of \citet{goebel2012hybrid} as a means of certifying the safety of hybrid systems. In the hybrid automata modeling framework \citep{lygeros2003dynamical}, such hybrid barrier functions have been proposed in \citet{prajna2007framework}.

The underlying challenge and bottleneck in verifying safety using barrier functions and ensuring (by appropriate control action) safety using control barrier functions is the construction of even these functions.  The authors in \citet{prajna2007framework} propose a sum-of-squares programming approach for finding polynomial (hybrid) barrier functions for polynomial (hybrid) systems and semi-algebraic sets. For finding CBFs, sum-of-squares programming and analytic approaches have been presented in \citet{ames2019control,xu2017correctness}, and \citet{wang2018permissive} which, however, only apply to specific systems and have limited scalability. In \citet{yaghoubi2020training}, a deep neural network is trained to imitate the control law obtained from a CBF. The authors in \citet{srinivasan2020synthesis} synthesize a CBF from safe and unsafe data samples using support vector machines. In \citet{saveriano2019learning}, the authors cluster observed data and learn a linear CBFs for each cluster.  While the aforementioned works \citep{yaghoubi2020training,srinivasan2020synthesis,saveriano2019learning} present detailed empirical validation of their methods, no formal correctness proofs are provided. In \citet{ferlez2020shieldnn}, a way to learn a provably correct neural net safety guards for kinematic bicycle models is presented. The authors in \citet{jin2020neural} propose a method to provably learn a control barrier function and the corresponding control law. Readily available data in the form of state-input observation pairs are, however, not used and the authors instead rely on solving nested min-max optimization problems. Also related to our work is \citet{giesl2019approximation} where a function is learned that approximates an underlying Lyapunov function. In \citet{robey2020learning}, a data-driven approach for learning CBFs has been presented by assuming knowledge of the system dynamics as well as availability of observed data illustrating safe behavior of the system. This paper also provides sufficient conditions that ensure the correctness of the learned CBFs using a Lipschitz argument.

\textbf{Contributions: } First, for a class of hybrid control systems with some mild regularity assumptions, we present \emph{hybrid control barrier functions} as a means to enforce forward invariance of a safe set. We in particular provide sufficient conditions in terms of a HCBF that, if satisfied by a control law, ensure safety. Second, we formulate the problem of learning HCBFs from data as a constrained optimization problem and provide conditions under which a feasible solution is a HCBF.  Third, we present exhaustive simulation studies to showcase the proposed framework. 


==> chapter/simulations.tex <==
\section{Case Studies}
\label{sec:case_studies}

The code for both case studies is provided in the supplementary material.
%
In both our simulations, we numerically
integrate the hybrid dynamics of interest using an integrator implementation inspired by
Drake~\citep{drake}. We build our implementation on top of
\texttt{scipy.integrate.solve\_ivp}'s 
event detection API. This allows us to 
get precise notifications for when a system makes
a discrete jump.

\paragraph{Bouncing ball}
Our first experiment considers the controlled bouncing ball discussed in Example \ref{ex:2}.
Here we use a safe set $\mathcal{S}$ with a velocity bound $\zeta = 2$.
The parameter $\gamma$ is set to be the gravitational acceleration, i.e. $\gamma = 9.81$.
We generate expert data for this system as follows.
We first create a reference path shown as dash-dotted blue lines in Figure \ref{fig:ball}. The reference path in the left half plane is generated by dropping the ball at $(1,0)$ without applying any control input  until it hits the ground.
The discrete input $u_d$ is set to $1.0$ when the collision happens.
Then reversing the velocity in sign gives the reference path in the right half plane.
We then design a linear error-feedback control law $u_{c,\text{nom}} = K (z(t,j)-z_{\text{ref}}(t))$ with $K = \begin{bmatrix} 10, 5.48 \end{bmatrix}$ via solving the Riccati equation in order to track the reference during the continuous flow.
The reference state $z_{\text{ref}}(t)$ is found by nearest neighbour search.
We set the nominal discrete input to be $u_{d,\text{nom}} = 1.2$ such that it amplifies the velocities after collisions and thus is more likely to cause constraint violation.
Note that neither the reference path nor the closed-loop trajectory obtained by applying the nominal controller $u_{c,\text{nom}}$ complies with the safe set $\mathcal{S}$.
Next, we implement the analytical HCBF in Example \ref{ex:2}, which, per solving of the CBF-QP problem \citet{ames2014control}, gives a safe controller $u_{c,\text{safe}}$ during flow.
The safe control input $u_{d,\text{safe}}$ 
during jump is essentially a thresholding function and can be found analytically as mentioned in Example \ref{ex:2}.
Using the above controllers, we obtain data-sets $Z^c_{\text{safe}}$ and $Z^d_{\text{safe}}$ containing 5000 safe states and associated expert demonstrations $u^i_c$ and $u^i_d$.
Those expert states, shown as the green and magenta dots in the left subplot of Figure \ref{fig:ball}, are evenly gridded near the boundary of the safe set $\mathcal{S}$.
We in addition fine-grid 1140 unsafe samples on the boundary of $\mathcal{N}$ to form the data-set $Z_N$.
To better shape the learned HCBF, we adopt the control barrier filter idea proposed in \citet{robey2020learning} by gridding 2500 safe samples in int$(\mathcal{S})$.
% The training data is plotted in Figure \ref{fig:ball}.

We parametrize the HCBF candidate $h$ with a two-hidden-layer fully-connected deep neural network (DNN). The DNN uses tanh activation functions and has 32 neurons in each hidden layer. The training is implemented using jax \citet{bradbury2020jax} and the Adam algorithm with a cosine decay learning rate. 
We craft a loss function by relaxing the constraints in \eqref{eq:opt}.
See \citet{robey2020learning} for details regarding this relaxation procedure.
We then train the DNN for $10^5$ epochs with hyperparameters 
$\gamma_\text{safe} = 0.05$, $\gamma_\text{unsafe}=0.5$, $\gamma_\text{dyn}^c = 1.5$ and $\gamma_\text{dyn}^d = 1.5$ chosen via grid-search.
The set $\mathcal{C}$ of the learned HCBF is shown as green dots in the middle subplot of Figure \ref{fig:ball}.
One may clearly observe that $\mathcal{C}$ is strictly contained within the geometric safe set, i.e. $\mathcal{C} \subset \mathcal{S}$.

\begin{figure}[h!]
\centering
% \includegraphics[scale=0.56]{ball.pdf}
\includegraphics[scale=0.56]{ball.png}
\caption{Left: Plot of the expert states $Z^c_{\text{safe}}$ (green) and $Z^d_{\text{safe}}$ (magenta), safe samples (blue) and unsafe samples $Z_\mathcal{N}$ (red). Dashed red lines indicate bounds on the velocity.
Middle: Closed-loop simulation of the bouncing ball using the learned HCBF where the initial state, state before jump, state after jump and terminal state are indicated by a red diamond, magenta star, magenta circle and red cross, respectively. The solid black line and dashed blue line represent the closed-loop and reference path. The green dots represent the set $\mathcal{C}=\{z\in\mathbb{R}^{n_z} \, \big{|} \, h(z)\ge 0\}$ where $h$ is the learned HCBF.
Right: Closed-loop simulation of the bouncing ball using the analytical HCBF.}
\label{fig:ball}
\end{figure}

We now test if the learned HCBF is able to produce safe control input that keeps the system within the set $\mathcal{C}$.
We consider the same setup as in the expert demonstration. 
Note again that applying the nominal control law $u_{c,\text{nom}}$ alone would lead to violation of the velocity constraint.
Starting from an initial state $(0.1, -1.8)$, we simulate the controlled system for $2.2$ seconds.
During flow, we solve the CBF-QP problem for the continuous input $u_{c,\text{safe}}$.
During jump, we perform line search with a decay factor $\rho = 0.95$ to find the scalar discrete input $u_{d,\text{safe}}$ that satisfies \eqref{eq:cbf_disc_hybrid}.
The closed-loop trajectory produced by the learned HCBF is plotted in Figure \ref{fig:ball}.
As a comparison, we also plot the trajectory obtained using the analytical HCBF in Example \ref{ex:2}.
Albeit being a little conservative comparing to the analytical HCBF, the learned HCBF manages to keep the state within $\mathcal{C}$ at all times during both flow and jump.

\paragraph{Compass gait}

\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{phase_portrait.png}
    \end{subfigure} \quad
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{walker_guy.png}
    \end{subfigure}
    \caption{Caption}
    \label{fig:compass-gait}
\end{figure}

In this section, we consider a more challenging setting: learning a hybrid control barrier function for the compass gait walker \citep{goswami1996limit,byl2008approximate}.  Originally introduced by Goswami et al.\ in \citep{goswami1996limit}, the compass gait dynamics describe the motion of a passive bipedal robot walking down an inclined plane at a constant velocity.  This system uses a four dimension state, which describes the angle and angular veloctiy for each of the two legs.  For conciseness, we detail these dynamics in the appendix and provide further background for the compass gait walker in the Appendix \textcolor{red}{[]}.

To collect expert trajectories in this setting, we simulate the compass gait system with an energy-based controller detailed in \citep{goswami1997limit}; see Appendix \textcolor{red}{[]} for details.  Learning and analyzing a HCBF for this system proposes several challenges, which include the well-known sensitivity of the compass gait walker to its initial conditions and the inherent difficulties in visualizing a four-dimensional state space.  Thus to simplify our approach, when collecting expert trajectories, we fix the initial condition for the angle and angular velocity of the left leg to be a point $[0, 0.4]$ on the passive limit cycle; we then vary the initial condition of the right leg by adding uniform noise to corresponding passive limit cycle state $[0, 2.0]$ for the right leg.

As in the previous case study, we parameterize the candidate HCBF $h$ with a two-hidden-layer fully-connected neural network with tanh activations; as before, we determine the hyperpameters by grid search.  However, unlike the previous example, the task of identifying boundary points is complicated by the higher dimensionality of the state space.  Therefore, we propose a novel algorithm that can be used to identify boundary points by sampling from the space of expert trajectories.  In essence, the algorithm, which is fully characterized in Appendix \textcolor{red}{X}, identifies boundary points by computing the pairwise distances between all of the expert states and thresholding based on these distances.

In the left panel of Figure \ref{fig:compass-gait}, we show a visualization of the learned HCBF.  In particular, starting from an initial condition with the same left leg state as the expert trajectories, we identify the values for $h(x)$ at which $u_{\text{CBF}} - u_{\text{nom}} > 0$ in green, i.e. where the CBF controller takes over the nominal controller.  In red, we plot the phase portrait for the right leg corresponding to a trajectory using the HCBF-QP controller.  To demonstrate the physical interpretation of this learned CBF, in the right panel of Figure \ref{fig:compass-gait}, we show the motion of the compass gait walker down the ramp, marking in green where the CBF-based controller takes over.

\begin{algorithm}
    \centering
    \begin{algorithmic}[1]
        \Statex \textbf{Input: } Tuple of $d$-dimensional vectors $X := \{x_1, \dots, x_n\}$, minimum number of neighbors $N\in\mathbb{Z}_+$, neighbor threshold $\eta > 0$
        \Statex \textbf{Output: } Binary vector $\{y_1, \dots, y_n\} \subset \{0, 1\}^n$
        \Statex
        \State $M \gets compute\_pairwise\_dists(X)$ \quad\# compute pairwise distances between vectors in $X$
        \State $\tilde{M}_{i,j} \gets M_{i,j} \cdot \mathbbm{1}(M_{i,j} \leq \eta)$ for $i,j\in\{1, \dots, n\}$ \quad\# threshold $M$ by $\eta$
        \State $\tilde{y} \gets sum(\tilde{M}, \text{axis}=1)$ \quad\# sum across the columns of $\tilde{M}$
        \State $y \gets \mathbbm{1}(\tilde{y} \leq N)$ \quad\# threshold $\tilde{y}$ by $N$
    \end{algorithmic}
    \caption{Mr.\ Peanut}
    \label{alg:mr-peanut}
\end{algorithm}

